Dimensionwise Separable 2-D Graph Convolution for Unsupervised and Semi-Supervised Learning on Graphs

Graph convolutional neural networks (GCN) have been the model of choice for graph representation learning, which is mainly due to the effective design of graph convolution that computes the representation of a node by aggregating those of its neighbors. However, existing GCN variants commonly use 1-D graph convolution that solely operates on the object link graph without exploring informative relational information among object attributes. This significantly limits their modeling capability and may lead to inferior performance on noisy and sparse real-world networks. In this paper, we explore 2-D graph convolution to jointly model object links and attribute relations for graph representation learning. Specifically, we propose a computationally efficient dimensionwise separable 2-D graph convolution (DSGC) for filtering node features. Theoretically, we show that DSGC can reduce intra-class variance of node features on both the object dimension and the attribute dimension to learn more effective representations. Empirically, we demonstrate that by modeling attribute relations, DSGC achieves significant performance gain over state-of-the-art methods for node classification and clustering on a variety of real-world networks. The source code for reproducing the experimental results is available at https://github.com/liqimai/DSGC.

==> biography.tex <==
% biography section
%
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Bio/QimaiLi}}]{Qimai Li}
	is currently a Ph.D. student at the Department of Computing, the Hong Kong Polytechnic University, supervised by Dr. Wu Xiao-Ming. He obtained B.Eng. degree from the College of Computer Science and Technology, Zhejiang University. His main area of interest includes machine learning on graph, semi-supervised Learning and graph signal processing. He publishes in leading venues including CVPR, EMNLP, IJCAI and AAAI.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Bio/XiaotongZhang}}]{Xiaotong Zhang}
  is an associate research professor in the School of Software, Dalian University of Technology. She received the B.Eng. degree in software engineering and the Ph.D. degree in computer application technology from Dalian University of Technology in 2012 and 2018 respectively. Before she joined in Dalian University of Technology, she worked as a postdoctoral fellow in the Department of Computing, The Hong Kong Polytechnic University. She has published over 20 papers on journals and conferences, including TKDE, TKDD, Neural Networks, KBS, ACL, EMNLP, CVPR, IJCAI, AAAI, etc. Her research interests include machine learning, artificial intelligence and data mining.
\end{IEEEbiography}

\vfill

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Bio/HanLiu}}]{Han Liu}
  is currently an associate professor in the School of Software, Dalian University of Technology. He received the B.Eng. degree in software engineering and the Ph.D. degree in computer application technology from Dalian University of Technology in 2012 and 2018 respectively. Before he joined in Dalian University of Technology, he worked as a postdoctoral fellow in the Department of Computing, The Hong Kong Polytechnic University. He has published over 20 papers on journals and conferences, including TKDE, TKDD, Neural Networks, KBS, ACL, EMNLP, CVPR, IJCAI, AAAI, etc. His research interests include machine learning, artificial intelligence and data mining.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Bio/QuanyuDai}}]{Quanyu Dai}
	received the B.Eng. degree from the Department of Electronic Engineering, Shanghai Jiao Tong University, Shanghai, China, in 2015. He is now a Ph.D. candidate at the Department of Computing, The Hong Kong Polytechnic University, Hong Kong. His research interests include representation learning, transfer learning, deep learning, and adversarial learning for graph-structured data. He has publications appeared in the top-tier conferences and journals, such as IJCAI, AAAI and WWW.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/Bio/Xiao-MingWu}}]{Xiao-Ming Wu}
	is currently an assistant professor at the Department of Computing, The Hong Kong Polytechnic University. She works on machine learning and artificial intelligence. Her research has contributed to new theoretical insights of machine learning algorithms and novel methods for artificial intelligence applications in various fields. She publishes in leading venues including NeurIPS, CVPR, EMNLP, IJCAI and AAAI. She obtained her PhD degree from the Department of Electrical Engineering, Columbia University in 2016. Prior to that, she obtained her MPhil Degree from the Chinese University of Hong Kong and her bachelor’s and master’s degrees from Peking University.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks
